Low Rank Matrix Completion with Exponential Family Noise

The matrix completion problem consists in reconstructing a matrix from a sample of entries, possibly observed with noise. A popular class of estimator, known as nuclear norm penalized estimators, are based on minimizing the sum of a data fitting term and a nuclear norm penalization. Here, we investigate the case where the noise distribution belongs to the exponential family and is sub-exponential. Our framework alllows for a general sampling scheme. We first consider an estimator defined as the minimizer of the sum of a log-likelihood term and a nuclear norm penalization and prove an upper bound on the Frobenius prediction risk. The rate obtained improves on previous works on matrix completion for exponential family. When the sampling distribution is known, we propose another estimator and prove an oracle inequality w.r.t. the Kullback-Leibler prediction risk, which translates immediatly into an upper bound on the Frobenius prediction risk. Finally, we show that all the rates obtained are minimax optimal up to a logarithmic factor.

==> abstract.tex <==
\begin{abstract}
The task of reconstructing a matrix given a sample of observed
entries is known as the \emph{matrix completion problem}. Such a consideration arises in
a wide variety of problems, including recommender systems, collaborative
filtering, dimensionality reduction, image processing, quantum physics or multi-class classification
to name a few. Most works have focused on recovering an unknown real-valued low-rank
matrix from randomly sub-sampling its entries.
Here, we investigate the case where the observations take a finite numbers of values, 
corresponding for examples to ratings in 
recommender systems or labels in multi-class classification.
We also consider a general sampling scheme (non-necessarily uniform) over the matrix entries.
The performance of a nuclear-norm penalized estimator is analyzed theoretically.
More precisely, we derive bounds for the Kullback-Leibler divergence between the true and estimated distributions.
In practice,  we have also proposed an efficient algorithm based on lifted coordinate gradient descent in order to tackle
potentially high dimensional settings.
\end{abstract}


==> defs.tex <==
documentclass[12pt]{article}
% Retirez le caractere "%" au debut de la ligne ci--dessous si votre
% editeur de texte utilise des caracteres accentues
% \usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
%
% Retirez le caractere "%" au debut des lignes ci--dessous si vous
% utiisez les symboles et macros de l'AMS
% \usepackage{amsmath}
% \usepackage{amsfonts}
%
\usepackage{amsmath,amsthm,amstext,amsfonts,amssymb}
\usepackage{dsfont}
\usepackage{mathrsfs}

\usepackage{mathrsfs}
\usepackage{enumerate}
\usepackage{hyperref}
\usepackage{bbm}
\usepackage{showlabels}
